Trade-offs between membership privacy & adversarially robust learning

Historically, machine learning methods have not been designed with security in mind. In turn, this has given rise to adversarial examples, carefully perturbed input samples aimed to mislead detection at test time, which have been applied to attack spam and malware classification, and more recently to attack image classification. Consequently, an abundance of research has been devoted to designing machine learning methods that are robust to adversarial examples. Unfortunately, there are desiderata besides robustness that a secure and safe machine learning model must satisfy, such as fairness and privacy. Recent work by Song et al. (2019) has shown, empirically, that there exists a trade-off between robust and private machine learning models. Models designed to be robust to adversarial examples often overfit on training data to a larger extent than standard (non-robust) models. If a dataset contains private information, then any statistical test that separates training and test data by observing a model's outputs can represent a privacy breach, and if a model overfits on training data, these statistical tests become easier. In this work, we identify settings where standard models will overfit to a larger extent in comparison to robust models, and as empirically observed in previous works, settings where the opposite behavior occurs. Thus, it is not necessarily the case that privacy must be sacrificed to achieve robustness. The degree of overfitting naturally depends on the amount of data available for training. We go on to characterize how the training set size factors into the privacy risks exposed by training a robust model on a simple Gaussian data task, and show empirically that our findings hold on image classification benchmark datasets, such as CIFAR-10 and CIFAR-100.

==> parts/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\noindent \textbf{Relationship with adversarial examples.} Ostensibly, a weakness of this work is that the robust optimization procedure creates examples that should be classified differently by an oracle classifier, and so the term ``adversarial examples'' is a misnomer. 
We fully agree with the general point that this analysis blurs of the meaning of ``adversarial examples'', however in our analysis we do not make any claims surrounding ground-truth classification of adversarial examples. 
Indeed, we are entirely uninterested in adversarial examples in this work; what we are concerned with is how robust optimization procedures (such as adversarial training) affect other desirable properties of a classifier, such as privacy (resistance to membership inference attacks).
Of course, we relate privacy to the $\epsilon$ used during the robust optimization procedure, but we are not interested in the robust generalization error, as was the main focus in \citet{tsipras2018there} and 
\citet{tsipras2018robustness} -- we are interested solely in two properties, standard error and privacy. 
Interestingly, in the Gaussian model, standard error fell to zero for even very large $\epsilon$ values, and so it is fair to measure these models with equivalent test set accuracy, in terms of their privacy. 

We show in \cref{fig:cifar10_mem_inf_train_vs_size} that $\epsilon$ does not need to be large to train models that are more private than standard models. For example, using a CIFAR-10 training set of size between 200-500, and setting $\epsilon=\frac{8}{255}$ -- which is small enough that perturbed inputs will maintain their ground-truth semantic label -- the robust models are more resistant to privacy attacks than standard models. Thus, in practice, we do not need to use a large $\epsilon$ to inherit this privacy property in robust models. Translating our theory from a Gaussian setting to more interesting distributions to study this property in more detail is an interesting direction for future work. 

